RAG-based User Profiling for Precision Planning in Mixed-precision Over-the-Air Federated Learning

Mixed-precision computing, a widely applied technique in AI, offers a larger trade-off space between accuracy and efficiency. The recent purposed Mixed-Precision Over-the-Air Federated Learning (MP-OTA-FL) enables clients to operate at appropriate precision levels based on their heterogeneous hardware, taking advantages of the larger trade-off space while covering the quantization overheads in the mixed-precision modulation scheme for the OTA aggregation process. A key to further exploring the potential of the MP-OTA-FL framework is the optimization of client precision levels. The choice of precision level hinges on multifaceted factors including hardware capability, potential client contribution, and user satisfaction, among which factors can be difficult to define or quantify. In this paper, we propose a RAG-based User Profiling for precision planning framework that integrates retrieval-augmented LLMs and dynamic client profiling to optimize satisfaction and contributions. This includes a hybrid interface for gathering device/user insights and an RAG database storing historical quantization decisions with feedback. Experiments show that our method boosts satisfaction, energy savings, and global model accuracy in MP-OTA-FL systems.

==> old.tex <==

Over-the-air federated learning (OTA-FL) has recently emerged as a promising approach for efficient model aggregation across large networks of distributed clients. To extend this paradigm to heterogeneous user devices, we previously introduced mixed-precision OTA-FL (MP-OTA-FL) allowing clients with heterogeneous hardware to operate at suitable precision levels. In real-world applications, selecting optimal precision levels that maximize the user satisfaction levels in MP-OTA-FL hinges on multifaceted factors, including both intrinsic technical ones that are easy to quantify and extrinsic contextual ones that are difficult to enumerate.

Considering this, we propose a user-in-the-loop precision planning framework that synergizes retrieval-augmented large language models (LLMs) with dynamic client profiling to optimize user satisfaction and their contribution. The framework consists of a hybrid conversational interface that collects knowledge from both the device and the user and a RAG knowledge database that stores historical quantization decision-making with user feedback. Experimental results demonstrate that our approach enhances user satisfaction while improving resource utilization and energy efficiency in mixed-precision OTA-FL systems.

deterministic parameters and an LLM-driven chat agent to iteratively uncover latent usage patterns and environmental context.
The synthesized data informs a benefit-cost matrix that quantifies precision options against user experience metrics (accuracy, latency) and resource costs (energy, bandwidth). These matrices drive an adaptive quantization allocator that strategically distributes precision levels across clients under fixed communication budgets.

Recognizing the heterogeneous nature of input factors—where hardware constraints and explicit preferences (e.g., latency tolerance) can be directly specified, while operational contexts (e.g., network stability) and usage habits (e.g., app engagement frequency) require nuanced exploration—
while improving resource utilization efficiency by 26% and reducing energy waste by 41%, outperforming static and heuristic precision selection baselines.
The selection of operating precision for clients is a key to optimizing the framework for model performance, resource utilization, and user satisfaction. For a single client, the optimal precision is determined by a preset target performance or delay, which can vary among users with different preferences and can change over time.

In this paper, we propose a novel solution to automate and optimize this precision selection process by leveraging a retrieval-augmented large language model. Our method fuses device specification (e.g., power state, processing power), model quantization benchmark, with user-provided inputs obtained via a chat-based survey (e.g., application usage patterns, performance expectation, delay tolerance) to produce a benefit-cost matrix for each user, quantifying how each available precision option affects user experience and resource consumption. These matrices guide a quantization scheme that adapts the distribution of precision levels among selected clients for a given communication resource budget. 

% \begin{itemize}
%     \item \textbf{Limitations in user preference modeling}: Traditional approaches use preset targets, but users have heterogeneous satisfaction criteria across performance, delay, and energy consumption that significantly impact optimal quantization decisions.
    
%     \item \textbf{Challenges in measuring client contribution}: Direct measurement is infeasible due to data privacy in FL, leading to reliance on proxy metrics and heuristics with inherent approximation errors.
% \end{itemize}


% The framework leverages a RAG-LLM to interpret usage, user preferences, operation environment from chat-based survey inputs of open end questions. And then combining information directly read from client devices such as hardware specifications, retrieve the best matching quantization level for the client from user case knowledge base. 


% \item We propose a novel RAG-LLM-based human-centric quantization planning framework for mixed-precision OTA-FL systems, which incorporates user preferences and resource constraints to optimize user satisfaction and FL performance.
% \item We demonstrate the effectiveness of the proposed framework through a mixed-precision FL voice assistant system in terms of user satisfaction and resource consumption.





% \section{Discussion}

% \subsection{Advantages}

% Our proposed RAG-based precision planning framework effectively addresses the challenges identified in mixed-precision OTA-FL systems. By combining retrieval-augmented LLMs with dynamic profiling, we achieved higher user satisfaction, better resource allocation, and improved overall efficiency compared to baseline methods.

% \subsection{Limitations}

% Despite promising results, our method has several limitations:

% \begin{itemize} \item \textbf{Generalization and Robustness of LLM}: While RAG-LLM effectively handles common cases, performance for outlier user preferences and contexts may degrade. More targeted fine-tuning on domain-specific datasets could further enhance robustness. \item \textbf{Computational Overhead}: Integrating RAG-LLM introduces computational overhead, especially critical on resource-constrained client devices. Further optimization and offloading computations onto server-side components might mitigate these concerns. \item \textbf{Dependence on Quality of User Feedback}: The effectiveness of the proposed approach heavily relies on accurate and honest user feedback. Inconsistent or malicious feedback could negatively impact system performance. \end{itemize}

% \subsection{Future Directions}

% Future research could address the limitations and further enhance our framework by:

% \begin{itemize} \item Exploring lightweight RAG-LLM models suitable for deployment on resource-constrained edge devices. \item Developing robust feedback aggregation and filtering strategies to ensure the integrity of the knowledge database. \item Extending the approach to handle multi-objective optimization dynamically, potentially employing reinforcement learning for adaptive preference management. \item Investigating privacy-preserving user feedback collection mechanisms integrated within RAG-based systems. \end{itemize}
